A Fully Spiking Hybrid Neural Network for Energy-Efficient Object Detection

This paper proposes a Fully Spiking Hybrid Neural Network (FSHNN) for energy-efficient and robust object detection in resource-constrained platforms. The network architecture is based on Convolutional SNN using leaky-integrate-fire neuron models. The model combines unsupervised Spike Time-Dependent Plasticity (STDP) learning with back-propagation (STBP) learning methods and also uses Monte Carlo Dropout to get an estimate of the uncertainty error. FSHNN provides better accuracy compared to DNN based object detectors while being 150X energy-efficient. It also outperforms these object detectors, when subjected to noisy input data and less labeled training data with a lower uncertainty error.

==> Extras/motivation.tex <==
\section{Motivation}
In this section, we discuss the primary motivation for using a hybrid spiking based object detector. We discuss the energy advantages and the generalization advantages we can get by fusing the features learned using STDP with the SGD process.

\subsubsection{Energy Advantage for Spiking Neural Networks}
 Spiking Neural Networks are widely used instead of standard Artificial Neural Networks to improve the energy-efficiency of the DNNs. This energy-efficiency arises since the standard ANNs communicate using continuous-valued activations while SNNs offer an opportunity using spike events that are sparse in time. Presently, efficacious training of standard ANNs requires the use of energy-intensive high-end graphic cards. On the other hand, in Spiking networks the output spike trains can be made sparse in time. An advantage of this in biological networks is that the spike events consume energy and that using few spikes which have high information content reduces energy consumption \cite{stone2018principles}. This same advantage perpetuates in the hardware \cite{merolla2014million, seo201145nm, carrillo2012advancing}. Thus, it is possible to create low energy spiking hardware based on the property that spikes are sparse in time.

% Horowitz et. al. \cite{horowitz20141} showed that a 32-bit floating-point (FL) MAC operation consumes 4.6 pJ(0.9 + 3.7 pJ) and 0.9 pJ for an AC operation. A 32-bit integer (INT) MAC operation consumes 3.2 pJ (0.1 + 3.1 pJ) and 0.1 pJ for an AC operation. Based on these measures, we calculated the energy consumption of the spiking object detectors by multiplying FLOPS (floating-point operations)and the energy consumption of MAC and AC operations calculated. The FLOPS for the different architectures described in the paper is tabulated in Table \ref{tab:energy} shows that FSHNN and the other spiking object detectors demonstrate exceptional energy efficiency for 32-bit FL and INT operations.



\subsubsection{Transfer Learning and Feature Fusion:}
 Here we motivate the use of feature fusion using STDP and SGD for object detection. It is based on the fact that features learned using the STDP learning procedure can complement the standard neural network and make the training easier, more generalizable, and robust. Zeiler et al. used tools of visualization, the authors observed that the lower layers converged much faster compared to the higher layers \cite{zeiler2014visualizing}. Also, they claimed that small transformations in the input image have a larger effect on the lower layers compared to the higher layers. Again, some recent works have empirically shown that a convolutional network trained on a large dataset can be successfully generalized to other tasks where less data is available \cite{donahue2014decaf}. These observations motivated us to use additional layers in the initial stages of the backbone classifier to capture the low-level features. 
Donahue et al. showed that lower level features can be very transferred to different networks to get superior performance \cite{yosinski2014transferable}. Developing on these ideas, we utilize the pre-trained spiking convolutional layers trained using the unsupervised STDP method since it can better apprehend local features that are independent of the dataset compared to the standard DNN. Also since STDP trained layers are robust to noise and can train with fewer unlabelled training data samples, it is a better choice.
In addition to this, Jacot et al. showed that the generalizability of an infinitely wide neural network is dependent on the initialization and a better initialization also improves the generalizability of the network \cite{jacot2018neural}. 
Thus, we show the generalizability of the STDP process compared to the standard SGD which would subsequently prove the spiking architecture to have better generalizability characteristics as compared to its DNN counterpart.

\subsection{Generalizability of STDP}
We compare the generalization bounds of a spiking convolutional neural network to its DNN counterpart considering the same architecture.
Considering STDP based learning method for the spiking network while the SGD based one for DNN, we study the Hausdorff dimension of the trajectories of the two learning methodologies as shown in \cite{csimcsekli2020hausdorff}. 
The authors demonstrated that the generalization error can be controlled by the uniform Hausdorff dimension of the learning algorithm, along with the constants inherited from the regularity conditions. The authors also showed that the generalization error can be controlled by the tail behavior of the process with heavier-tails implying less generalization error.

Now, recent literature has shown that STDP based learning in spiking neural networks follow an Ornstein–Uhlenbeck process \cite{leen2012approximating} as compared to SGD which follows the Feller process \cite{simsekli2020hausdorff}. So, we now aim to compare the heavy-tailed nature of the two processes by comparing the tail indices. 

We use stochastic differential equations (SDEs) to formulate local plasticity rules for parameters $\theta_{i}$ that control synaptic connections (if $\left.\theta_{i}>0\right)$ and synaptic weights $w_{i}=\exp \left(\theta_{i}-\theta_{0}\right)$
\begin{align}
d \theta_{i}=\left(b \frac{\partial}{\partial \theta_{i}} \log p^{*}(\boldsymbol{\theta})\right) d t+\sqrt{2 T b} \cdot d \mathcal{W}_{i} \nonumber \\ \text { where } d \mathcal{W}_{i} \text { denotes an infinitesimal }
\end{align}
step of a random walk (Wiener process), drift diffusion $\mathrm{b}=$ learning rate, $\mathrm{T}=$ temperature (T=1 until last slide)

The Fokker-Planck (FP) equation tracks the resulting evolution of the spiking network configurations $\boldsymbol{\theta}$ over time, yielding the stationary distribution $\frac{1}{z}p^*(\boldsymbol{\theta})^{1/T}$ which follows the Ornstein–Uhlenbeck process \cite{leen2012approximating}
\begin{align}
\frac{\partial}{\partial t} p_{F P}(\boldsymbol{\theta}, t)=\sum_{i}-\frac{\partial}{\partial \theta_{i}}\left(\left(b \frac{\partial}{\partial \theta_{i}} \log p^{*}(\boldsymbol{\theta})\right) p_{F P}(\boldsymbol{\theta}, t)\right) \nonumber \\ + \frac{\partial^{2}}{\partial \theta_{i}^{2}}\left(T b p_{F P}(\boldsymbol{\theta}, t)\right)
\end{align}

 Now, the practically relevant forms of the target distribution $p^*(\boldsymbol{\theta})$ of network configurations depend on the type of learning. For this case, we consider the unsupervised learning method described in 
\cite{kappel2015synaptic}.
Now, we perform a tail index analysis of STDP in deep spiking neural networks, similar to the method adopted in \cite{simsekli2019tail}. 









\textbf{Method for tail-index estimation:} A wide plethora of works have delved into the matter of estimating the tail-index of an extreme-value distribution. \cite{de1998comparison, dekkers1989moment, hill1975simple, pickands1975statistical}. However, since most of these methods fail to estimate the tail index of $\alpha$-stable distributions \cite{mittnik1996tail, paulauskas2011once}, the estimator method is described as follows:


\begin{theorem} \cite{mohammadi2015estimating}
 Let $\left\{X_{i}\right\}_{i=1}^{K}$ be a collection of random variables with $X_{i} \sim \mathcal{S} \alpha \mathcal{S}(\sigma)$ and $K=K_{1} \times K_{2} .$ Define $Y_{i} \triangleq \sum_{j=1}^{K_{1}} X_{j+(i-1) K_{1}}$ for $i \in\left[1, K_{2}\right] .$ Then, the estimator
\begin{align}
\widehat{\frac{1}{\alpha}} \triangleq \frac{1}{\log K_{1}}\left(\frac{1}{K_{2}} \sum_{i=1}^{K_{2}} \log \left|Y_{i}\right|-\frac{1}{K} \sum_{i=1}^{K} \log \left|X_{i}\right|\right)
\label{eq:estimator}
\end{align}
converges to $1 / \alpha$ almost surely, as $K_{2} \rightarrow \infty$.
\end{theorem}
As shown in \cite{mohammadi2015estimating}, this estimator admits a faster convergence rate and smaller asymptotic variance than the aforementioned methods.


In order to estimate the tail-index $\alpha$ at iteration $k,$ we first partition the set of data points $\mathcal{D} \triangleq\{1, \ldots, n\}$ into many disjoint sets $\Omega_{k}^{i} \subset \mathcal{D}$ of size $b,$ such that the union of these subsets give all the data points. Formally, for all $i, j=1, \ldots, n / b,\left|\Omega_{k}^{i}\right|=b, \cup_{i} \Omega_{k}^{i}=\mathcal{D},$ and $\Omega_{k}^{i} \cap \Omega_{k}^{j}=\emptyset$ for $i \neq j$
% This approach is similar to sampling without replacement.
We then compute the full gradient $\nabla f\left(\mathbf{w}_{k}\right)$ and the stochastic gradients $\nabla \tilde{f}_{\Omega_{k}^{i}}\left(\mathbf{w}_{k}\right)$ for each minibatch $\Omega_{k}^{i} .$ Finally. we compute the stochastic gradient noises $U_{k}^{i}\left(\mathbf{w}_{k}\right)=\nabla \tilde{f}_{\Omega_{i}}\left(\mathbf{w}_{k}\right)-\nabla f\left(\mathbf{w}_{k}\right),$ vectorize each $U_{k}^{i}\left(\mathbf{w}_{k}\right)$ and concatenate
them to obtain a single vector, and compute the reciprocal of the estimator given in Eq. \ref{eq:estimator}. We use $K=p n / b$ and $K_{1}$ is the divisor of $K$ that is the closest to $\sqrt{K}$ for our experiments.

Similar to the analysis done by \cite{simsekli2019tail}, we evaluate the tail-index of the CNN and the SCNN networks trained with the SGD and the frequency-dependent STDP processes respectively. The experiment is repeated with varying numbers of layers and is evaluated on the MNIST dataset and the tail indices are reported in Table \ref{tab:tail}. We observe that the STDP process has a smaller value of $\alpha$ for each of the cases thus implying that the distribution has a heavier tail and thus is more generalizable.


\begin{table}[]
\centering
\caption{Comparison of Tail Indices $\alpha$ of SGD, STDP for varying depth in Convolutional Networks\cite{simsekli2019tail}}
\label{tab:tail}
\resizebox{0.47\columnwidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}No. of\\ Layers\end{tabular}} & \textbf{SGD} & \textbf{STDP} \\ \hline
\textbf{3} & 1.297 & 1.206 \\ \hline
\textbf{4} & 1.291 & 1.193 \\ \hline
\textbf{5} & 1.284 & 1.188 \\ \hline
\textbf{6} & 1.273 & 1.181 \\ \hline
\end{tabular}%
}
\end{table}



Since STDP is more generalizable than SGD, this motivates us to utilize both these methods by introducing a model that fuses the STDP and the SGD based learning methods.

==> Extras/perf_eval.tex <==
\section{Experiments}

In this section, we discuss the experiments performed and the results obtained when testing our novel fully spiking hybrid neural network architecture. First, we evaluate the performance of the proposed architecture with respect to the ablation studies on the MS-COCO dataset \cite{lin2014microsoft}. Following that, we repeat the experiment for different input noise levels and evaluate the performance of the model. Similarly, we also evaluated the performance of the model on limited labelled datasets. Finally, we also evalaute the energy efficiency of the model compared to the standard object detection methods.
MS COCO dataset, with 223K frames that contain instances  from 81 different  object  categories,  and  an official 118K/5K training/testing split. 

\subsection{Evaluation Metrics:}

The two main evaluation metrics that are used to quantify the performance of object detectors discussed above are:
\begin{enumerate}

    \item  \textbf{Mean Average Precision $(m A P):$} is an accepted metric for evaluating object detection performance. $\mathrm{mAP}$ measures a detector's ability to detect all objects in a closed set dataset with a correct classification and accurate localization $(\mathrm{IoU} \geq 0.5),$ while minimizing incorrect detections and their confidence score. A perfect mAP score is $100 \%$ For performance on the detection task, we use the Mean Average Precision (mAP) at 0.5 IOU. The maximum mean average precision achievable by a detector is $100 \%$.

\item  \textbf{Uncertainty Error (UE)} \cite{harakeh2020bayesod}, \cite{miller2019evaluating}: This metric represents the ability of an uncertainty measure to accept correct detections and reject incorrect detections. The uncertainty error, defined in Eq.\ref{eq:UE}, is the probability that a detection is incorrectly accepted or rejected at a given uncertainty threshold $(\delta),$ i.e. the proportion of correct detections $D_{c}$ that are incorrectly rejected and the proportion of incorrect detections $\mathbb{D}_{i}$ that are incorrectly accepted.
\begin{equation}
    U E(\delta)=0.5 \frac{\left|U\left(\mathbb{D}_{c}\right)>\delta\right|}{\left|\mathbb{D}_{c}\right|}+0.5 \frac{\left|U\left(\mathbb{D}_{i}\right) \leq \delta\right|}{\left|\mathbb{D}_{i}\right|}
    \label{eq:UE}
\end{equation}

The minimum uncertainty error represents the ideal threshold for separating correct and incorrect detections and the highest uncertainty effectiveness achievable by a detector. This metric weights the probability of correct detections and incorrect detections equally.
The Minimum Uncertainty Error (MUE) at 0.5 IOU is used to determine the ability of the detector's estimated uncertainty to discriminate true positives from false positives. The lowest MUE achievable by a detector is $0 \% .$ We define the Categorical MUE (CMUE) as we are using the Categorical entropy and finally, we average the CMUE over all categories in a testing dataset to arrive to a single value, the Mean (Categorical) MUE (mCMUE).
\end{enumerate}




% Finally, we use the newly proposed Probability Based Detection Quality (PDQ) [27] to jointly quantify the bounding box and category probability assigned to true positives by the detector. The highest PDQ achievable by a detector is $100 \%$, where  the  PDQ  increases  as  the  distributions  assigned  to  a detection  better  match  those  of  the  ground  truth  instance.




\subsection{Performance Evaluation of FSHNN}

In this section, we evaluate the performance of the FSHNN based object detetor on the MS-COCO dataset. We do so by performing three separate experiments. First, we evaluate the performance of the model under normal circumstances, trained with all the input data and tested with clean images. We repeat this experiment for multiple STDP layers in the \textbf{Block 2}, as shown in Fig. \ref{fig:block1}.

From Table \ref{tab:abl1}, we see that the inclusion of more STDP layers improves the classification loss to a greater extent than the regression loss. Also, inclusion of more layers make the network more robust, but at the cost of increased parameters and hence energy consumption. However, it must be noted here that the training of the STDP layers is unsupervised and thus this step does not require any labelled data.
\begin{table*}[]
\centering
\caption{Table showing Performance of the FSHNN based Object Detector with Increasing STDP Layers}
\label{tab:abl1}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c||c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}No. of \\ STDP\\ Layers\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Classifi-\\ cation\\  Loss\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Regres-\\ sion \\ Loss\end{tabular}} & \textbf{mAP} & \textbf{AP}_S & \textbf{AP}_M & \textbf{AP}_L & \textbf{mAR} & \textbf{AR}_S & \textbf{AR}_M & \textbf{AR}_L  & \textbf{mCMUE}\\ \hline 

\textbf{3}                                                               & 0.4127                                                                      & 0.6912                                                                  & 0.379  & &  &     & 0.492    & & &  & 0.251 \\ \hline
\textbf{4}                                                               & 0.3841                                                                      & 0.6787                                                                  & 0.392  & &  &    & 0.515    & & &   & 0.244 \\ \hline
\textbf{5}                                                               & 0.3352                                                                      & 0.6536                                                                  & 0.409    & & &   & 0.527   & & &    & 0.236 \\ \hline
\textbf{6}                                                               & 0.3076                                                                      & 0.6193                                                                  & 0.426   & &  &   & 0.541    & &  &  & 0.229 \\ \hline
\end{tabular}
\end{table*}




\subsection{ Performance with Input Noise in Testing}
We evaluate the average precision and recall of the proposed FSHNN based object detector. The model is tested on the MS-COCO dataset under three different scenarios: 1. with no noise 2. with signal to noise ratio (S.N.R) = 30dB and 3. with signal to noise ratio (S.N.R) = 15dB. The results of the experiments are summarized in Table \ref{tab:abl2}. We see that with increasing noise level, the spiking based object detector outperforms the DNN based object detectors by larger margins. This highlights the fact that FSHNN based object detectors are more robust to noise than their DNN counterparts.

% We further test the robustness of the model by testing the model with different adversarial conditions - first we use two different noise levels (SNR = 30dB , 15dB) and also evaluate the performance after training the model with increasingly limited labelled data (80\%, 60\% and 40\% data respectively).
% These results are summarized in Tables \ref{tab:abl1}, \ref{tab:abl2}. 

% In this section, we evaluate the performance of the STDP layers in the object detection algorithm. We have trained models with different number of STDP layers and evaluated the classification and regression loss for the same. Hence, we have subjected each of the architectures with noisy data and less labelled data to study the effect that the STDP layers on these adversarial conditions.

% From Table \ref{tab:abl1}, we see that the inclusion of more STDP layers improves the classification loss to a greater extent than the regression loss. Also, inclusion of more layers make the network more robust, but at the cost of increased parameters and hence energy consumption. However, it must be noted here that the training of the STDP layers is unsupervised and thus this step does not require any labelled data.

\subsubsection{Performance after Training with Less Data}
We also evaluated our model by training it with lesser amount of data. Previously, \cite{panda2017convolutional} has shown that using a Convolutional SNN requires lesser amount of data when compared to the fully connected SNN. In this work, we compare the performance of the back propagated SNN with the hybrid SNN model for object detection tasks. We train the model on a partial MS COCO dataset and reported the average precision and recall. We see that increasing the number of STDP layers greatly improves the performance of the FSHNN based object detector especially when the amount of data removed is significant. Thus, we may conclude that the STDP layers which were trained with unlabelled data learns features which are critical in the classification problem as can be seen from the falling classification loss with increasing STDP layers in Table \ref{tab:abl2}.




\begin{table}[]
\centering
\caption{Table showing Robustness of FSHNN based Object Detector for Noisy Testing Data and Limited Labelled Training Dataset }
\label{tab:abl2}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}No. of \\ STDP\\ Layers\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Classifi-\\ cation\\  Loss\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Regres-\\ sion \\ Loss\end{tabular}} & \textbf{mAP} & \textbf{mAR} & \tetbf{cMUE}  \\ \hline
\multicolumn{6}{|c|}{\textbf{SNR = 30dB}}                                                                                                                                                                                                                              \\ \hline
\textbf{3}                                                               & 0.4318                                                                      & 0.7165                                                                  & 0.368        & 0.483        & 0.317 \\ \hline
\textbf{4}                                                               & 0.3987                                                                      & 0.7093                                                                  & 0.382        & 0.497        & 0.305 \\ \hline
\textbf{5}                                                               & 0.3516                                                                      & 0.6845                                                                  & 0.395        & 0.519        & 0.291 \\ \hline
\textbf{6}                                                               & 0.3204                                                                      & 0.6522                                                                  & 0.412        & 0.531        & 0.284 \\ \hline
\multicolumn{6}{|c|}{\textbf{SNR = 15dB}}                                                                                                                                                                                                                              \\ \hline
\textbf{3}                                                               & 0.6723                                                                      & 0.7345                                                                  & 0.305        & 0.441        & 0.455 \\ \hline
\textbf{4}                                                               & 0.6552                                                                      & 0.7269                                                                  & 0.316        & 0.453        & 0.448 \\ \hline
\textbf{5}                                                               & 0.6218                                                                      & 0.7114                                                                  & 0.324        & 0.465        & 0.439 \\ \hline
\textbf{6}                                                               & 0.6014                                                                      & 0.7008                                                                  & 0.331        & 0.476        & 0.431 \\ \hline
\hline
\multicolumn{6}{|c|}{\textbf{80\% Training Data}}                                                                                                                                                                                                                               \\ \hline
\textbf{3}                                                               & 0.4157                                                                      & 0.6998                                                                  & 0.358        & 0.473        & 0.301 \\ \hline
\textbf{4}                                                               & 0.3806                                                                      & 0.6742                                                                  & 0.363        & 0.481        & 0.289 \\ \hline
\textbf{5}                                                               & 0.3694                                                                      & 0.6516                                                                  & 0.392        & 0.514        & 0.214 \\ \hline
\textbf{6}                                                               & 0.3356                                                                      & 0.6288                                                                  & 0.411        & 0.547        & 0.199 \\ \hline
\multicolumn{6}{|c|}{\textbf{60\% Training Data}}                                                                                                                                                                                                                               \\ \hline
\textbf{3}                                                               & 0.4975                                                                      & 0.7884                                                                  & 0.329        & 0.431        & 0.390 \\ \hline
\textbf{4}                                                               & 0.4698                                                                      & 0.7545                                                                  & 0.348        & 0.476        & 0.358 \\ \hline
\textbf{5}                                                               & 0.4513                                                                      & 0.7312                                                                  & 0.364        & 0.493        & 0.317 \\ \hline
\textbf{6}                                                               & 0.4027                                                                      & 0.7084                                                                  & 0.396        & 0.518        & 0.296 \\ \hline
\multicolumn{6}{|c|}{\textbf{40\% Training Data}}                                                                                                                                                                                                                               \\ \hline
\textbf{3}                                                               & 0.6057                                                                      & 0.9432                                                                  & 0.287        & 0.386        & 0.513 \\ \hline
\textbf{4}                                                               & 0.5964                                                                      & 0.9303                                                                  & 0.296        & 0.401        & 0.501 \\ \hline
\textbf{5}                                                               & 0.5837                                                                      & 0.9268                                                                  & 0.308        & 0.415        & 0.486 \\ \hline
\textbf{6}                                                               & 0.5759                                                                      & 0.9115                                                                  & 0.322        & 0.426        & 0.478 \\ \hline
\end{tabular}
\end{table}




% \begin{table}[]
% \centering
% \caption{Table showing Ablation Studies with increasing number of STDP layers for varying noise levels}
% \label{tab:my-table}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}No. of \\ STDP\\ Layers\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Classifi-\\ cation\\  Loss\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Regres-\\ sion \\ Loss\end{tabular}} & \textbf{mAP} & \textbf{mAR} & \tetbf{cMUE}  \\ \hline
% \multicolumn{6}{|c|}{\textbf{No Noise}}                                                                                                                                                                                                                                \\ \hline
% \textbf{3}                                                               & 0.4127                                                                      & 0.6912                                                                  & 0.379        & 0.492        & 0.251 \\ \hline
% \textbf{4}                                                               & 0.3841                                                                      & 0.6787                                                                  & 0.392        & 0.515        & 0.244 \\ \hline
% \textbf{5}                                                               & 0.3352                                                                      & 0.6536                                                                  & 0.409        & 0.527        & 0.236 \\ \hline
% \textbf{6}                                                               & 0.3076                                                                      & 0.6193                                                                  & 0.426        & 0.541        & 0.229 \\ \hline
% \multicolumn{6}{|c|}{\textbf{SNR = 30dB}}                                                                                                                                                                                                                              \\ \hline
% \textbf{3}                                                               & 0.4318                                                                      & 0.7165                                                                  & 0.368        & 0.483        & 0.317 \\ \hline
% \textbf{4}                                                               & 0.3987                                                                      & 0.7093                                                                  & 0.382        & 0.497        & 0.305 \\ \hline
% \textbf{5}                                                               & 0.3516                                                                      & 0.6845                                                                  & 0.395        & 0.519        & 0.291 \\ \hline
% \textbf{6}                                                               & 0.3204                                                                      & 0.6522                                                                  & 0.412        & 0.531        & 0.284 \\ \hline
% \multicolumn{6}{|c|}{\textbf{SNR = 15dB}}                                                                                                                                                                                                                              \\ \hline
% \textbf{3}                                                               & 0.6723                                                                      & 0.7345                                                                  & 0.305        & 0.441        & 0.455 \\ \hline
% \textbf{4}                                                               & 0.6552                                                                      & 0.7269                                                                  & 0.316        & 0.453        & 0.448 \\ \hline
% \textbf{5}                                                               & 0.6218                                                                      & 0.7114                                                                  & 0.324        & 0.465        & 0.439 \\ \hline
% \textbf{6}                                                               & 0.6014                                                                      & 0.7008                                                                  & 0.331        & 0.476        & 0.431 \\ \hline
% \end{tabular}
% \end{table}























\subsection{Performance Comparison with Baselines}

In this section, we test the performance of the model with different baselines. We have selected two bsaelines models for this comparison which are described as follows:
\begin{enumerate}
    \item \textbf{Retinanet:} Retinanet is a state-of-the-art DNN based object detector which works using the Focal Pyramid Network architecture. The 
        \item \textbf{Back Propagated Fully Spiking Object Detector: }For the back propagated fully spiking retinanet we replace the STDP layers (\texttt{Block 1} in Fig \ref{fig:block1}) in the FSHNN based object detector with corresponding DNN layers. For this experiment, we have replaced 3 STDP layers with 3 Convolution Layers. Hence, we use a similar DNN-to-SNN conversion methodology to obtain a Fully Spiking Object Detector which has backpropagated spiking layers with the same architecture as FSHNN based object detector. With the weights obtained in this conversion process as initialization point, we retrain the model using STBP to get the final trained model. 
\end{enumerate}

We perform a two-fold evaluation of the FSHNN model with the baselines described above - first we evaluate the performance of the object detectors without any perturbation and trained with the full training dataset. The results are shown in Fig. \ref{tab:perf_comp}. We see that though the FSHNN with 3 STDP layers performs closely to the Retinanet, the FSHNN with 6 STDP layers outperforms the Retinanet with respect to both mAP/mAR and uncertainty error.

We test the robustness of the model by testing the model with different adversarial conditions - first we use two different noise levels (SNR = 30dB , 15dB) and also evaluate the performance after training the model with increasingly limited labelled data (80\%, 60\% and 40\% data respectively).

 We observe that in the no noise scenario, the FSHNN with 6 STDP layers outperforms the Retinanet and the difference in their performances increase as the input noise level is increased or the model is trained with lesser amount of labelled data. This highlights the fact that the spiking neural networks are more robust to input noise and perturbations when compared to the standard neural networks. 





% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table*}[]
% \caption{No Noise}
% \label{tab:my-table}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{1}{|l|}{}                                                                     & \textbf{AP} & \textbf{APS} & \textbf{APM} & \textbf{APL} & \textbf{AR} & \textbf{ARS} & \textbf{ARM} & \textbf{ARL} \\ \hline
% \textbf{RetinaNet 101}                                                                     & 0.388       & 0.207        & 0.420        & 0.498        & 0.501       & 0.301        & 0.566        & 0.624        \\ \hline
% \textbf{FSHNN Obj Det (converted)}                                                         & 0.379       & 0.198        & 0.407        & 0.482        & 0.492       & 0.292        & 0.554        & 0.615        \\ \hline
% \textbf{FSHNN Obj Det 101}                                                                 & 0.349       & 0.169        & 0.368        & 0.461        & 0.435       & 0.257        & 0.493        & 0.580        \\ \hline
% \textbf{SAFE-DNN Obj Det 101}                                                              & 0.386       & 0.209        & 0.417        & 0.491        & 0.502       & 0.305        & 0.561        & 0.626        \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking Obj Detector 101\\ (converted)\end{tabular}} & 0.375       & 0.189        & 0.401        & 0.477        & 0.486       & 0.283        & 0.549        & 0.598        \\ \hline
% \end{tabular}%
% }
% \end{table*}

% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table}[]
% \caption{SNR = 30dB}
% \label{tab:my-table}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{1}{|l|}{}                                                                     & \textbf{AP} & \textbf{APS} & \textbf{APM} & \textbf{APL} & \textbf{AR} & \textbf{ARS} & \textbf{ARM} & \textbf{ARL} \\ \hline
% \textbf{RetinaNet 101}                                                                     & 0.371       & 0.183        & 0.409        & 0.481        & 0.489       & 0.279        & 0.554        & 0.613        \\ \hline
% \textbf{FSHNN Obj Det (converted)}                                                         & 0.368       & 0.190        & 0.395        & 0.476        & 0.483       & 0.285        & 0.549        & 0.605        \\ \hline
% \textbf{SAFE-DNN Obj Det 101}                                                              & 0.373       & 0.188        & 0.408        & 0.476        & 0.488       & 0.283        & 0.551        & 0.610        \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking Obj Detector 101\\ (converted)\end{tabular}} & 0.365       & 0.186        & 0.388        & 0.472        & 0.478       & 0.278        & 0.543        & 0.589        \\ \hline
% \end{tabular}%
% }
% \end{table}

% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table}[]
% \caption{SNR = 15dB}
% \label{tab:my-table}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{1}{|l|}{}                                                                     & \textbf{AP} & \textbf{APS} & \textbf{APM} & \textbf{APL} & \textbf{AR} & \textbf{ARS} & \textbf{ARM} & \textbf{ARL} \\ \hline
% \textbf{RetinaNet 101}                                                                     & 0.277       & 0.104        & 0.237        & 0.349        & 0.416       & 0.204        & 0.401        & 0.426        \\ \hline
% \textbf{FSHNN Obj Det (converted)}                                                         & 0.305       & 0.163        & 0.358        & 0.417        & 0.441       & 0.257        & 0.496        & 0.573        \\ \hline
% \textbf{SAFE-DNN Obj Det 101}                                                              & 0.281       & 0.106        & 0.240        & 0.351        & 0.419       & 0.207        & 0.402        & 0.429        \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking Obj Detector 101\\ (converted)\end{tabular}} & 0.297       & 0.159        & 0.347        & 0.406        & 0.428       & 0.248        & 0.473        & 0.559        \\ \hline
% \end{tabular}%
% }
% \end{table}


\begin{table*}[]
\centering
\caption{Table showing the performance of the different object detectors}
\label{tab:perf_comp}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c||c|}
\hline
% \multicolumn{9}{|c|}{\textbf{mAP}}   \multicolumn{2}{|c|}{\textbf{UE}}                 \\ \hline
& \textbf{mAP} & \textbf{AP}_S & \textbf{AP}_M & \textbf{AP}_L & \textbf{mAR} & \textbf{AR}_S & \textbf{AR}_M & \textbf{AR}_L  & \textbf{mCMUE}\\ \hline
\multicolumn{10}{|c|}{\textbf{No Noise; 100\% Training Data}}                                                                                                                                                           \\ \hline
\textbf{RetinaNet}                                                          & 0.388       & 0.207        & 0.420        & 0.498        & 0.501       & 0.301        & 0.566        & 0.624    &  0.237    \\ \hline

% \textbf{SAFE-DNN Obj Det}                                                   & 0.386       & 0.209        & 0.417        & 0.491        & 0.502       & 0.305        & 0.561        & 0.626       & 0.243   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.375       & 0.189        & 0.401        & 0.477        & 0.486       & 0.283        & 0.549        & 0.598      &  0.254   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                      & 0.379       & 0.198        & 0.407        & 0.482        & 0.492       & 0.292        & 0.554        & 0.615     & 0.251   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                      &    0.426    &     0.223    &   0.452      &   0.526      &   0.541     &   0.312      &    0.611     &   0.682   &  0.229  \\ \hline
\end{tabular}%
}
\end{table*}










\begin{table*}[]
\centering
\caption{Table showing the performance of the different object detectors with input noise during testing}
\label{tab:comp_noise}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c||c|}
\hline
% \multicolumn{9}{|c|}{\textbf{mAP}}   \multicolumn{2}{|c|}{\textbf{UE}}                 \\ \hline
& \textbf{mAP} & \textbf{AP}_S & \textbf{AP}_M & \textbf{AP}_L & \textbf{mAR} & \textbf{AR}_S & \textbf{AR}_M & \textbf{AR}_L  & \textbf{mCMUE}\\ \hline

\multicolumn{10}{|c|}{\textbf{SNR = 30dB}}                                                                                                                                                         \\ \hline
\textbf{RetinaNet}                                                          & 0.371       & 0.183        & 0.409        & 0.481        & 0.489       & 0.279        & 0.554        & 0.613   & 0.313  \\ \hline

% \textbf{SAFE-DNN Obj Det}                                                   & 0.373       & 0.188        & 0.408        & 0.479        & 0.488       & 0.283        & 0.551        & 0.610     & 0.309   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.365       & 0.186        & 0.388        & 0.472        & 0.478       & 0.278        & 0.543        & 0.589       & 0.320 \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                      & 0.368       & 0.190        & 0.395        & 0.476        & 0.483       & 0.285        & 0.549        & 0.605       & 0.317   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                      &  0.412      &   0.211      &   0.446      &       0.482  &     0.531   &  0.308       &  0.599        &    0.668    &  0.284  \\ \hline
\multicolumn{10}{|c|}{\textbf{SNR = 15dB}}                                                                                                                                                         \\ \hline
\textbf{RetinaNet}                                                          & 0.277       & 0.104        & 0.237        & 0.349        & 0.416       & 0.204        & 0.401        & 0.426       & 0.605  \\ \hline

% \textbf{\begin{tabular}[c]{@{}c@{}}SAFE-DNN \\ Obj Det\end{tabular}}        & 0.281       & 0.106        & 0.240        & 0.351        & 0.419       & 0.207        & 0.402        & 0.429       & 0.601  \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.297       & 0.159        & 0.347        & 0.406        & 0.428       & 0.248        & 0.473        & 0.539       & 0.483  \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                     & 0.305       & 0.163        & 0.358        & 0.417        & 0.441       & 0.257        & 0.496        & 0.553     & 0.455   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                    &   0.331     &   0.184      &    0.392     &   0.451      &    0.476     &    0.271    &    0.528     &  0.587    &  0.431  \\ \hline

\end{tabular}%
}
\end{table*}











\begin{table*}[]
\centering
\caption{Table showing the performance of the different object detectors with input noise during testing}
\label{tab:comp_data}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c||c|}
\hline
% \multicolumn{9}{|c|}{\textbf{mAP}}   \multicolumn{2}{|c|}{\textbf{UE}}                 \\ \hline
& \textbf{mAP} & \textbf{AP}_S & \textbf{AP}_M & \textbf{AP}_L & \textbf{mAR} & \textbf{AR}_S & \textbf{AR}_M & \textbf{AR}_L  & \textbf{mCMUE}\\ \hline

% \multicolumn{10}{|c|}{\textbf{SNR = 30dB}}                                                                                                                                                         \\ \hline
% \textbf{RetinaNet}                                                          & 0.371       & 0.183        & 0.409        & 0.481        & 0.489       & 0.279        & 0.554        & 0.613   & 0.313  \\ \hline

% % \textbf{SAFE-DNN Obj Det}                                                   & 0.373       & 0.188        & 0.408        & 0.479        & 0.488       & 0.283        & 0.551        & 0.610     & 0.309   \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.365       & 0.186        & 0.388        & 0.472        & 0.478       & 0.278        & 0.543        & 0.589       & 0.320 \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                      & 0.368       & 0.190        & 0.395        & 0.476        & 0.483       & 0.285        & 0.549        & 0.605       & 0.317   \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                      &  0.412      &   0.211      &   0.446      &       0.482  &     0.531   &  0.308       &  0.599        &    0.668    &  0.284  \\ \hline
% \multicolumn{10}{|c|}{\textbf{SNR = 15dB}}                                                                                                                                                         \\ \hline
% \textbf{RetinaNet}                                                          & 0.277       & 0.104        & 0.237        & 0.349        & 0.416       & 0.204        & 0.401        & 0.426       & 0.605  \\ \hline

% % \textbf{\begin{tabular}[c]{@{}c@{}}SAFE-DNN \\ Obj Det\end{tabular}}        & 0.281       & 0.106        & 0.240        & 0.351        & 0.419       & 0.207        & 0.402        & 0.429       & 0.601  \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.297       & 0.159        & 0.347        & 0.406        & 0.428       & 0.248        & 0.473        & 0.539       & 0.483  \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                     & 0.305       & 0.163        & 0.358        & 0.417        & 0.441       & 0.257        & 0.496        & 0.553     & 0.455   \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                    &   0.331     &   0.184      &    0.392     &   0.451      &    0.476     &    0.271    &    0.528     &  0.587    &  0.431  \\ \hline

% \hline 
\multicolumn{10}{|c|}{\textbf{80\% training set}}                                                                                                                                                  \\ \hline
\textbf{RetinaNet}                                                          & 0.376       & 0.189        & 0.398        & 0.478        & 0.481       & 0.287        & 0.543        & 0.608     &  0.308  \\ \hline

\textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.353       & 0.178        & 0.379        & 0.460        & 0.468       & 0.264        & 0.525        & 0.574      &   0.305 \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                      & 0.358       & 0.182        & 0.386        & 0.466        & 0.473       & 0.274        & 0.538        & 0.591      & 0.301   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                      & 0.411       & 0.221        & 0.452        & 0.521        & 0.547       & 0.311        & 0.594        & 0.662      & 0.199   \\ \hline
\multicolumn{10}{|c|}{\textbf{60\% training set}}                                                                                                                                                  \\ \hline
\textbf{RetinaNet}                                                          & 0.328       & 0.137        & 0.342        & 0.431        & 0.433       & 0.231        & 0.492        & 0.557      &  0.393  \\ \hline

\textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.316       & 0.129        & 0.328        & 0.424        & 0.423       & 0.221        & 0.476        & 0.541      &  0.396  \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                     & 0.329       & 0.140        & 0.341        & 0.435        & 0.431       & 0.235        & 0.488        & 0.552     & 0.390   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                     &   0.396     &    0.188     &   0.409      &   0.496      &    0.518    &   0.271      &    0.542     &   0.608   & 0.296   \\ \hline
\multicolumn{10}{|c|}{\textbf{40\% training set}}                                                                                                                                                  \\ \hline
\textbf{RetinaNet}                                                          & 0.234       & 0.056        & 0.266        & 0.351        & 0.349       & 0.158        & 0.413        & 0.472      & 0.799  \\ \hline

\textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.254       & 0.076        & 0.262        & 0.368        & 0.365       & 0.163        & 0.412        & 0.487     &  0.613  \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                     & 0.287       & 0.103        & 0.297        & 0.399        & 0.396       & 0.192        & 0.449        & 0.518   &  0.513  \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                     &   0.322     &   0.126      &   0.337      &  0.439      &       0.426  &    0.221    &   0.492      &  0.553  & 0.478   \\ \hline
% \multicolumn{10}{|c|}{\textbf{SNR = 10dB}}                                                                                                                                                         \\ \hline
% \textbf{RetinaNet}                                                          & 0.109       & 0.036        & 0.108        & 0.206        & 0.203       & 0.098        & 0.189        & 0.213       & 0.826  \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                       & 0.216       & 0.133        & 0.276        & 0.299        & 0.314       & 0.189        & 0.393        & 0.412      & 0.762   \\ \hline

% % \textbf{\begin{tabular}[c]{@{}c@{}}SAFE-DNN \\ Obj Det\end{tabular}}        & 0.161       & 0.093        & 0.175        & 0.274        & 0.289       & 0.174        & 0.257        & 0.288       & 0.799  \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.173       & 0.097        & 0.226        & 0.252        & 0.276       & 0.135        & 0.345        & 0.356      & 0.812   \\ \hline
\end{tabular}%
}
\end{table*}





















% \begin{table*}[]
% \centering
% \caption{Table showing the performance of the different object detectors with limited training data}
% \label{tab:training}
% \resizebox{0.7\textwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|c|c|c||c|}
% \hline
%                                                                             & \textbf{mAP} & \textbf{APS} & \textbf{APM} & \textbf{APL} & \textbf{mAR} & \textbf{ARS} & \textbf{ARM} & \textbf{ARL} & \textbf{mCMUE}\\ \hline
% \multicolumn{10}{|c|}{\textbf{80\% training set}}                                                                                                                                                  \\ \hline
% \textbf{RetinaNet}                                                          & 0.376       & 0.189        & 0.398        & 0.478        & 0.481       & 0.287        & 0.543        & 0.608     &  0.308  \\ \hline

% \textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.353       & 0.178        & 0.379        & 0.460        & 0.468       & 0.264        & 0.525        & 0.574      &   0.305 \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                      & 0.358       & 0.182        & 0.386        & 0.466        & 0.473       & 0.274        & 0.538        & 0.591      & 0.301   \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                      & 0.411       & 0.221        & 0.452        & 0.521        & 0.547       & 0.311        & 0.594        & 0.662      & 0.199   \\ \hline
% \multicolumn{10}{|c|}{\textbf{60\% training set}}                                                                                                                                                  \\ \hline
% \textbf{RetinaNet}                                                          & 0.328       & 0.137        & 0.342        & 0.431        & 0.433       & 0.231        & 0.492        & 0.557      &  0.393  \\ \hline

% \textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.316       & 0.129        & 0.328        & 0.424        & 0.423       & 0.221        & 0.476        & 0.541      &  0.396  \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                     & 0.329       & 0.140        & 0.341        & 0.435        & 0.431       & 0.235        & 0.488        & 0.552     & 0.390   \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                     &   0.396     &    0.188     &   0.409      &   0.496      &    0.518    &   0.271      &    0.542     &   0.608   & 0.296   \\ \hline
% \multicolumn{10}{|c|}{\textbf{40\% training set}}                                                                                                                                                  \\ \hline
% \textbf{RetinaNet}                                                          & 0.234       & 0.056        & 0.266        & 0.351        & 0.349       & 0.158        & 0.413        & 0.472      & 0.799  \\ \hline

% \textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.254       & 0.076        & 0.262        & 0.368        & 0.365       & 0.163        & 0.412        & 0.487     &  0.613  \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                     & 0.287       & 0.103        & 0.297        & 0.399        & 0.396       & 0.192        & 0.449        & 0.518   &  0.513  \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                     &   0.322     &   0.126      &   0.337      &  0.439      &       0.426  &    0.221    &   0.492      &  0.553  & 0.478   \\ \hline
% \end{tabular}%
% }
% \end{table*}




















\subsection{Energy Efficiency}
We also evaluate the energy efficiency of our spiking models with the standard ones and the results are given in Table \ref{tab:energy}. We see that the spiking neural network based object detector consumes significantly less power compared to the standard models, while giving comparable precision and recall. Firstly, most operations in DNNs occur in convolutional layers  where  the  multiply-accumulate  (MAC)  operations are primarily responsible during execution. SNNs, however,perform accumulate (AC) operations because spike events are  binary  operations  whose  input  is  integrated into  a  membrane  potential  only  when  spikes  are received. For a fair comparison, we focused solely on the computational power (MAC and AC) used to execute object detection on a single image. Horowitz et. al.  \cite{horowitz20141} showed that a 32-bit floating-point (FL) MAC operation consumes 4.6 pJ(0.9 + 3.7 pJ) and 0.9 pJ for an AC operation. A 32-bit integer (INT) MAC operation consumes 3.2 pJ (0.1 + 3.1 pJ) and 0.1 pJ for an AC operation. Based on these measures, we calculated the energy consumption of the spiking object detectors  by  multiplying  FLOPS  (floating-point  operations)and the energy consumption of MAC and AC operations calculated.The FLOPS for the different architectures described in the paper is given in Table \ref{tab:energy} shows that FSHNN and the other spiking object detectors demonstrates exceptional energy efficiency for 32-bit FL and INT operations.
 Total inference energy $E$ for ANN/SNN considering FLOPS count across all $N$ layers of a network is defined as \cite{panda2020toward}
$$
\begin{array}{l}
E_{A N N}=\left(\sum_{i=1}^{N} F L O P S_{A N N}\right) * E_{M A C} \\
E_{S N N}=\left(\sum_{i=1}^{N} F L O P S_{S N N}\right) * E_{A C} * T
\end{array}
$$
For SNN, the energy calculation considers the latency incurred as the rate-coded input spike train has to be presented over $T$ time-steps to yield the final prediction result. For this paper since we are using the STDB based approach to train the supervised SNN layers, we can get a high accuracy in 300 time steps. 


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Table showing the energy efficiency of spiking neural object detectors}
\label{tab:energy}
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
                                                                            & \textbf{Param(M)} & \textbf{FLOPS}       & \textbf{$EE = \frac{EE_{ANN}}{EE_{SNN}}$} \\ \hline
Retinanet                                                                   & 52.78             & $262.81 \times 10^9$ &                                           \\ \hline
\begin{tabular}[c]{@{}c@{}}SAFE-DNN\\  Obj Det\end{tabular}                 & 52.96             & $1.81 \times 10^8$   &                                           \\ \hline
\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Det\end{tabular}               & 52.99             & $1.85 \times 10^8$   & 151.53                                    \\ \hline
\begin{tabular}[c]{@{}c@{}}FSHNN \\ Obj Det \\ (3 layers STDP)\end{tabular} & 52.96             & $1.81 \times 10^8$   & 154.88                                    \\ \hline
\multicolumn{4}{|c|}{Ablation Studies}                                                                                                                             \\ \hline
\begin{tabular}[c]{@{}c@{}}FSHNN \\ Obj Det \\ (4 layers STDP)\end{tabular} & 53.04             & $1.84 \times 10^8$   & 152.35                                    \\ \hline
\begin{tabular}[c]{@{}c@{}}FSHNN \\ Obj Det \\ (5 layers STDP)\end{tabular} & 53.08             & $1.88 \times 10^8$   & 149.11                                    \\ \hline
\begin{tabular}[c]{@{}c@{}}FSHNN \\ Obj Det \\ (6 layers STDP)\end{tabular} & 53.11             & $1.90 \times 10^8$   & 147.54                                    \\ \hline
\end{tabular}%
}
\end{table}




\subsection{Comparison to Spiking Yolo}
{\color{red}
Spiking YOLO \cite{kim2020spiking} is the only spike based object detector in literature, so it is critical to check the performance difference between the two models. Though both the paper aim to solve the same problem, there are a few key differences in the two - firstly, the spiking yolo is based on YOLO architecture, which is generally used for real-time object detection tasks at the cost of precision and recall. However, the Retinanet model improves on the performance of the YOLO. Similarly, for the spiking object detectors proposed in this paper we see a significant increase in the observed mAP and mAR in MS-COCO dataset. While the spiking YOLO reported a mAP of 26.24\% , the FSHNN network described in this paper achieves $42.6\%$ which is extremely close to the mAP of the DNN based Retinanet object detector.  However, it must be noted that there is a significant difference in the architecture too - while the spiking yolo is based solely on the backpropagated Spiking convolution layers, the FSHNN uses both supervised backpropagation and unsupervised STDP based learning methods, giving a much higher accuracy than the spiking yolo. In addition to this, FSHNN also uses the MC Dropout method in order to calculate the uncertainty of the model, which further reinforces the robustness of the proposed architectural model.
 
However, it must also be noted that this comes at a cost - though our model has an energy advantage of around 150x compared to the DNN, it is comparatively larger to the Spiking YOLO network, which achieves a energy efficiency of 280x times the standard DNN.}

==> Extras/perf_eval_new.tex <==
\section{Experiments}

In this section, we present our experimental results using our novel FSHNN object detector compared to other spiking and non-spiking object detectors. First, we evaluate the performance of the proposed object detector on the MS-COCO dataset \cite{lin2014microsoft} with no adversarial conditions. Following that, we repeated the experiment by evaluating different input noise levels and also by training the models on limited labeled datasets. We compared the performance of our novel FSHNN based object detectors with the other baselines discussed in Section IV C. Finally, we also evaluated the energy efficiency of the models compared to the standard object detection methods.
For all the experiments we use the MS COCO dataset that has 223K frames with instances from 81 different object categories,  and a training/testing split of 118K/5K. 

\subsection{Evaluation Metrics:}

The two main evaluation metrics used to quantify the performance of object detectors discussed above are:
\begin{enumerate}

    \item  \textbf{Mean Average Precision $(m A P):$} is an accepted metric for evaluating object detection performance. $\mathrm{mAP}$ measures a detector's ability to detect all objects in a closed set dataset with a correct classification and accurate localization $(\mathrm{IoU} \geq 0.5),$ while minimizing incorrect detections and their confidence score. For performance on the detection task, we use the Mean Average Precision (mAP) at 0.5 IOU. The maximum mean average precision achievable by a detector is $100 \%$.

\item  \textbf{Uncertainty Error (UE)}  \cite{miller2019evaluating}: This metric represents the ability of an uncertainty measure to accept correct detections and reject incorrect detections. The uncertainty error, defined in Eq.\ref{eq:UE}, is the probability that a detection is incorrectly accepted or rejected at a given uncertainty threshold $(\delta),$ i.e. the proportion of correct detections $D_{c}$ that are incorrectly rejected and the proportion of incorrect detections $\mathbb{D}_{i}$ that are incorrectly accepted.
\begin{equation}
    U E(\delta)=0.5 \frac{\left|U\left(\mathbb{D}_{c}\right)>\delta\right|}{\left|\mathbb{D}_{c}\right|}+0.5 \frac{\left|U\left(\mathbb{D}_{i}\right) \leq \delta\right|}{\left|\mathbb{D}_{i}\right|}
    \label{eq:UE}
\end{equation}

The minimum uncertainty error represents the ideal threshold for separating correct and incorrect detections and the highest uncertainty effectiveness achievable by a detector. This metric equally weights the probability of correct and incorrect detections.
We use the Minimum Uncertainty Error (MUE) at 0.5 IOU to determine the ability of the detector's estimated uncertainty to discriminate true positives from false positives. The lowest MUE achievable by a detector is $0 \% .$ We define the Categorical MUE (CMUE) since we are using the Categorical entropy and finally, we average the CMUE overall categories in a testing dataset to derive the Mean (Categorical) MUE (mCMUE).
\end{enumerate}




\subsection{Performance Evaluation of FSHNN}

In this section, we evaluate the performance of the FSHNN based object detector on the MS-COCO dataset. We do so by performing three separate experiments. First, we evaluate the performance of the model under normal circumstances, train with all the input data, and test with clean images. We repeat this experiment for multiple STDP layers in the \textbf{Block 2}, as shown in Fig. \ref{fig:block1}. The results are summarized in Table  \ref{tab:abl1}.

From the table, we see that the inclusion of more STDP layers improves the classification loss to a greater extent than the regression loss. Also, the inclusion of more layers make the network more robust, but at the cost of increased parameters and hence energy consumption. However, it is to be noted that the training of the STDP layers is unsupervised and thus, this step does not require any labeled data.
\begin{table*}[]
\centering
\caption{Table showing Performance of the FSHNN based Object Detector with Increasing STDP Layers}
\label{tab:abl1}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c||c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}No. of \\ STDP\\ Layers\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Classifi-\\ cation\\  Loss\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Regres-\\ sion \\ Loss\end{tabular}} &  \textbf{mAP} & $\textbf{AP}_{S}$ & $\textbf{AP}_{M}$ & $\textbf{AP}_{L}$ & \textbf{mAR} & $\textbf{AR}_S$ & $\textbf{AR}_M$ & $\textbf{AR}_L$  & \textbf{mCMUE}\\ \hline 

\textbf{3}                                                               & 0.4127                                                                      & 0.6912                                                                  & 0.379  & 0.198 & 0.407 &  0.482   & 0.492    & 0.292 & 0.554 & 0.615  & 0.251 \\ \hline
\textbf{4}                                                               & 0.3841                                                                      & 0.6787                                                                  & 0.392  & 0.203 & 0.425 &  0.507  & 0.515    &  0.308 & 0.578 &  0.635 & 0.244 \\ \hline
\textbf{5}                                                               & 0.3352                                                                      & 0.6536                                                                  & 0.409    & 0.211 & 0.439 &  0.518 & 0.527   & 0.316 & 0.591 & 0.652   & 0.236 \\ \hline
\textbf{6}                                                               & 0.3076                                                                      & 0.6193                                                                  & 0.426   & 0.229 & 0.452 & 0.533  & 0.541    & 0.327 & 0.612 & 0.668 & 0.229 \\ \hline
\end{tabular}
\end{table*}




\subsubsection{ Performance with Input Noise in Testing}
We evaluate the average precision and recall of the proposed FSHNN based object detector on the MS-COCO dataset under three different scenarios: 1. with no noise 2. with the signal-to-noise ratio (S.N.R) = 30dB and 3. with the signal to noise ratio (S.N.R) = 15dB. The results of the experiments are summarized in Table \ref{tab:abl2}. We see that with increasing noise level, the spiking based object detector outperforms the DNN based object detectors by larger margins. This highlights the fact that FSHNN based object detectors are more robust to noise than their DNN counterparts.


\subsubsection{Performance after Training with Less Data}
We also evaluated our model by training it with a lesser amount of data.  We compare the performance of the hybrid SNN with the backpropagated SNN model and the non-spiking RetinaNet model for object detection tasks. We train the model on a partial MS COCO dataset and reported the average precision and recall. We see that increasing the number of STDP layers greatly improves the performance of the FSHNN based object detector especially when the amount of data removed is significant. Thus, we may conclude that the STDP layers which were trained with unlabelled data learn features that are critical in the classification problem as can be seen from the falling classification loss with increasing STDP layers in Table \ref{tab:abl2}.




\begin{table}[]
\centering
\caption{Table showing Robustness of FSHNN based Object Detector for Noisy Testing Data and Limited Labelled Training Dataset }
\label{tab:abl2}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}No. of \\ STDP\\ Layers\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Classifi-\\ cation\\  Loss\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Regres-\\ sion \\ Loss\end{tabular}} & \textbf{mAP} & \textbf{mAR} & \tetbf{cMUE}  \\ \hline
\multicolumn{6}{|c|}{\textbf{SNR = 30dB}}                                                                                                                                                                                                                              \\ \hline
\textbf{3}                                                               & 0.4318                                                                      & 0.7165                                                                  & 0.368        & 0.483        & 0.317 \\ \hline
\textbf{4}                                                               & 0.3987                                                                      & 0.7093                                                                  & 0.382        & 0.497        & 0.305 \\ \hline
\textbf{5}                                                               & 0.3516                                                                      & 0.6845                                                                  & 0.395        & 0.519        & 0.291 \\ \hline
\textbf{6}                                                               & 0.3204                                                                      & 0.6522                                                                  & 0.412        & 0.531        & 0.284 \\ \hline
\multicolumn{6}{|c|}{\textbf{SNR = 15dB}}                                                                                                                                                                                                                              \\ \hline
\textbf{3}                                                               & 0.6723                                                                      & 0.7345                                                                  & 0.305        & 0.441        & 0.455 \\ \hline
\textbf{4}                                                               & 0.6552                                                                      & 0.7269                                                                  & 0.316        & 0.453        & 0.448 \\ \hline
\textbf{5}                                                               & 0.6218                                                                      & 0.7114                                                                  & 0.324        & 0.465        & 0.439 \\ \hline
\textbf{6}                                                               & 0.6014                                                                      & 0.7008                                                                  & 0.331        & 0.476        & 0.431 \\ \hline
\hline
\multicolumn{6}{|c|}{\textbf{80\% Training Data}}                                                                                                                                                                                                                               \\ \hline
\textbf{3}                                                               & 0.4157                                                                      & 0.6998                                                                  & 0.358        & 0.473        & 0.301 \\ \hline
\textbf{4}                                                               & 0.3806                                                                      & 0.6742                                                                  & 0.363        & 0.481        & 0.289 \\ \hline
\textbf{5}                                                               & 0.3694                                                                      & 0.6516                                                                  & 0.392        & 0.514        & 0.214 \\ \hline
\textbf{6}                                                               & 0.3356                                                                      & 0.6288                                                                  & 0.411        & 0.547        & 0.199 \\ \hline
\multicolumn{6}{|c|}{\textbf{60\% Training Data}}                                                                                                                                                                                                                               \\ \hline
\textbf{3}                                                               & 0.4975                                                                      & 0.7884                                                                  & 0.329        & 0.431        & 0.390 \\ \hline
\textbf{4}                                                               & 0.4698                                                                      & 0.7545                                                                  & 0.348        & 0.476        & 0.358 \\ \hline
\textbf{5}                                                               & 0.4513                                                                      & 0.7312                                                                  & 0.364        & 0.493        & 0.317 \\ \hline
\textbf{6}                                                               & 0.4027                                                                      & 0.7084                                                                  & 0.396        & 0.518        & 0.296 \\ \hline
\multicolumn{6}{|c|}{\textbf{40\% Training Data}}                                                                                                                                                                                                                               \\ \hline
\textbf{3}                                                               & 0.6057                                                                      & 0.9432                                                                  & 0.287        & 0.386        & 0.513 \\ \hline
\textbf{4}                                                               & 0.5964                                                                      & 0.9303                                                                  & 0.296        & 0.401        & 0.501 \\ \hline
\textbf{5}                                                               & 0.5837                                                                      & 0.9268                                                                  & 0.308        & 0.415        & 0.486 \\ \hline
\textbf{6}                                                               & 0.5759                                                                      & 0.9115                                                                  & 0.322        & 0.426        & 0.478 \\ \hline
\end{tabular}
\end{table}
























\subsection{Performance Comparison with Baselines}

In this section, we test the performance of the model with different baselines. We have selected two baseline models for this comparison which are described as follows:
\begin{enumerate}
    \item \textbf{RetinaNet:} RetinaNet is a state-of-the-art DNN based object detector that works using the Focal Pyramid Network architecture. In this paper, we are using ResNet 101 as the backbone network for the RetinaNet object detector. 
        \item \textbf{Back Propagated Fully Spiking Object Detector: }For the backpropagated fully spiking RetinaNet we replace the STDP layers (\texttt{Block 1} in Fig \ref{fig:block1}) in the FSHNN based object detector with corresponding DNN layers. For this experiment, we have replaced 3 STDP layers with 3 Convolution Layers. Hence, we use a similar DNN-to-SNN conversion methodology to obtain a Fully Spiking Object Detector which has backpropagated spiking layers with the same architecture as FSHNN based object detector. With the weights obtained in this conversion process as the initialization point, we retrain the model using STBP to get the final trained model. 
\end{enumerate}

We perform a two-fold evaluation of the FSHNN model with the baselines described above - first we evaluate the performance of the object detectors without any perturbation and train with the full training dataset. The results are shown in Fig. \ref{tab:perf_comp}. We see that though the FSHNN with 3 STDP layers performs closely to the RetinaNet, the FSHNN with 6 STDP layers outperforms the RetinaNet with respect to both mAP/mAR and uncertainty error.

We test the robustness of the model by testing the model with different adversarial conditions - first, we use two different noise levels (SNR = 30dB, 15dB) and also evaluate the performance after training the model with increasingly limited labeled data (80\%, 60\%, and 40\% data respectively).

 We observe that in the no noise scenario, the FSHNN with 6 STDP layers outperforms the RetinaNet, and the difference in their performances increases as the input noise level is increased or the model is trained with a lesser amount of labeled data. This highlights the fact that the spiking neural networks are more robust to input noise and perturbations when compared to the standard neural networks. 







\begin{table*}[]
\centering
\caption{Table showing the performance of the different object detectors}
\label{tab:perf_comp}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c||c|}
\hline

& \textbf{mAP} & $\textbf{AP}_{S}$ & $\textbf{AP}_{M}$ & $\textbf{AP}_{L}$ & \textbf{mAR} & $\textbf{AR}_S$ & $\textbf{AR}_M$ & $\textbf{AR}_L$  & \textbf{mCMUE}\\ \hline
\multicolumn{10}{|c|}{\textbf{No Noise; 100\% Training Data}}                                                                                                                                                           \\ \hline
\textbf{RetinaNet}                                                          & 0.388       & 0.207        & 0.420        & 0.498        & 0.501       & 0.301        & 0.566        & 0.624    &  0.237    \\ \hline

\textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.375       & 0.189        & 0.401        & 0.477        & 0.486       & 0.283        & 0.549        & 0.598      &  0.254   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                      & 0.379       & 0.198        & 0.407        & 0.482        & 0.492       & 0.292        & 0.554        & 0.615     & 0.251   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                      &    0.426    &     0.223    &   0.452      &   0.526      &   0.541     &   0.312      &    0.611     &   0.682   &  0.229  \\ \hline
\end{tabular}%
}
\end{table*}










\begin{table*}[]
\centering
\caption{Table showing the performance of the different object detectors with input noise during testing}
\label{tab:comp_noise}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c||c|}
\hline

& \textbf{mAP} & $\textbf{AP}_{S}$ & $\textbf{AP}_{M}$ & $\textbf{AP}_{L}$ & \textbf{mAR} & $\textbf{AR}_S$ & $\textbf{AR}_M$ & $\textbf{AR}_L$  & \textbf{mCMUE}\\ \hline

\multicolumn{10}{|c|}{\textbf{SNR = 30dB}}                                                                                                                                                         \\ \hline
\textbf{RetinaNet}                                                          & 0.371       & 0.183        & 0.409        & 0.481        & 0.489       & 0.279        & 0.554        & 0.613   & 0.313  \\ \hline

\textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.365       & 0.186        & 0.388        & 0.472        & 0.478       & 0.278        & 0.543        & 0.589       & 0.320 \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                      & 0.368       & 0.190        & 0.395        & 0.476        & 0.483       & 0.285        & 0.549        & 0.605       & 0.317   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                      &  0.412      &   0.211      &   0.446      &       0.482  &     0.531   &  0.308       &  0.599        &    0.668    &  0.284  \\ \hline
\multicolumn{10}{|c|}{\textbf{SNR = 15dB}}                                                                                                                                                         \\ \hline
\textbf{RetinaNet}                                                          & 0.277       & 0.104        & 0.237        & 0.349        & 0.416       & 0.204        & 0.401        & 0.426       & 0.605  \\ \hline

\textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.297       & 0.159        & 0.347        & 0.406        & 0.428       & 0.248        & 0.473        & 0.539       & 0.483  \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                     & 0.305       & 0.163        & 0.358        & 0.417        & 0.441       & 0.257        & 0.496        & 0.553     & 0.455   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                    &   0.331     &   0.184      &    0.392     &   0.451      &    0.476     &    0.271    &    0.528     &  0.587    &  0.431  \\ \hline

\end{tabular}%
}
\end{table*}











\begin{table*}[]
\centering
\caption{Table showing the performance of the different object detectors with input noise during testing}
\label{tab:comp_data}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c||c|}
\hline
& \textbf{mAP} & $\textbf{AP}_{S}$ & $\textbf{AP}_{M}$ & $\textbf{AP}_{L}$ & \textbf{mAR} & $\textbf{AR}_S$ & $\textbf{AR}_M$ & $\textbf{AR}_L$  & \textbf{mCMUE}\\ \hline
\multicolumn{10}{|c|}{\textbf{80\% training set}}                                                                                                                                                  \\ \hline
\textbf{RetinaNet}                                                          & 0.376       & 0.189        & 0.398        & 0.478        & 0.481       & 0.287        & 0.543        & 0.608     &  0.308  \\ \hline

\textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.353       & 0.178        & 0.379        & 0.460        & 0.468       & 0.264        & 0.525        & 0.574      &   0.305 \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                      & 0.358       & 0.182        & 0.386        & 0.466        & 0.473       & 0.274        & 0.538        & 0.591      & 0.301   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                      & 0.411       & 0.221        & 0.452        & 0.521        & 0.547       & 0.311        & 0.594        & 0.662      & 0.199   \\ \hline
\multicolumn{10}{|c|}{\textbf{60\% training set}}                                                                                                                                                  \\ \hline
\textbf{RetinaNet}                                                          & 0.328       & 0.137        & 0.342        & 0.431        & 0.433       & 0.231        & 0.492        & 0.557      &  0.393  \\ \hline

\textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.316       & 0.129        & 0.328        & 0.424        & 0.423       & 0.221        & 0.476        & 0.541      &  0.396  \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                     & 0.329       & 0.140        & 0.341        & 0.435        & 0.431       & 0.235        & 0.488        & 0.552     & 0.390   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                     &   0.396     &    0.188     &   0.409      &   0.496      &    0.518    &   0.271      &    0.542     &   0.608   & 0.296   \\ \hline
\multicolumn{10}{|c|}{\textbf{40\% training set}}                                                                                                                                                  \\ \hline
\textbf{RetinaNet}                                                          & 0.234       & 0.056        & 0.266        & 0.351        & 0.349       & 0.158        & 0.413        & 0.472      & 0.799  \\ \hline

\textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.254       & 0.076        & 0.262        & 0.368        & 0.365       & 0.163        & 0.412        & 0.487     &  0.613  \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                     & 0.287       & 0.103        & 0.297        & 0.399        & 0.396       & 0.192        & 0.449        & 0.518   &  0.513  \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                     &   0.322     &   0.126      &   0.337      &  0.439      &       0.426  &    0.221    &   0.492      &  0.553  & 0.478   \\ \hline
\end{tabular}%
}
\end{table*}




































\subsection{Energy Efficiency}
We also evaluate the energy efficiency of our spiking models with the standard ones and the results are given in Table \ref{tab:energy}. We see that the spiking neural network-based object detector consumes significantly less power compared to the standard models while giving comparable precision and recall. Firstly, most operations in DNNs occur in convolutional layers where the multiply-accumulate  (MAC)  operations are primarily responsible during execution. SNNs, however, perform accumulate (AC) operations because spike events are binary operations whose input is integrated into a membrane potential only when spikes are received. For a fair comparison, we focused solely on computational power (MAC and AC) used to execute object detection on a single image. 

\par Horowitz et. al.  \cite{horowitz20141} showed that a 32-bit floating-point (FL) MAC operation consumes 4.6 pJ(0.9 + 3.7 pJ) and 0.9 pJ for an AC operation. A 32-bit integer (INT) MAC operation consumes 3.2 pJ (0.1 + 3.1 pJ) and 0.1 pJ for an AC operation. Based on these measures, we calculated the energy consumption of the spiking object detectors by multiplying  FLOPS  (floating-point operations)and the energy consumption of MAC and AC operations calculated. The FLOPS for the different architectures described in the paper is given in Table \ref{tab:energy} shows that FSHNN and the other spiking object detectors demonstrate exceptional energy efficiency for 32-bit FL and INT operations.
 Total inference energy $E$ for ANN/SNN considering FLOPS count across all $N$ layers of a network is defined as \cite{panda2020toward}
\begin{equation}
\begin{array}{l}
E_{A N N}=\left(\sum_{i=1}^{N} F L O P S_{A N N}\right) * E_{M A C} \\
E_{S N N}=\left(\sum_{i=1}^{N} F L O P S_{S N N}\right) * E_{A C} * T
\end{array}
\end{equation}
For SNN, the energy calculation considers the latency incurred as the rate-coded input spike train has to be presented over $T$ time-steps to yield the final prediction result. For this paper since we are using the STDB based approach to train the supervised SNN layers, we can get a high accuracy in 300 time steps. 


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Table showing the energy efficiency of spiking neural object detectors}
\label{tab:energy}
\resizebox{0.85\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
                                                                            & \textbf{Param(M)} & \textbf{FLOPS}       & \textbf{$EE = \frac{EE_{ANN}}{EE_{SNN}}$} \\ \hline
RetinaNet                                                                   & 52.78             & $262.81 \times 10^9$ &           N/A                                \\ \hline
% \begin{tabular}[c]{@{}c@{}}SAFE-DNN\\  Obj Det\end{tabular}                 & 52.96             & $1.81 \times 10^8$   &                                           \\ \hline
\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Det\end{tabular}               & 52.99             & $1.85 \times 10^8$   & 151.53                                    \\ \hline
\begin{tabular}[c]{@{}c@{}}FSHNN \\ Obj Det \\ (3 layers STDP)\end{tabular} & 52.96             & $1.81 \times 10^8$   & 154.88                                    \\ \hline
\multicolumn{4}{|c|}{Ablation Studies}                                                                                                                             \\ \hline
\begin{tabular}[c]{@{}c@{}}FSHNN \\ Obj Det \\ (4 layers STDP)\end{tabular} & 53.04             & $1.84 \times 10^8$   & 152.35                                    \\ \hline
\begin{tabular}[c]{@{}c@{}}FSHNN \\ Obj Det \\ (5 layers STDP)\end{tabular} & 53.08             & $1.88 \times 10^8$   & 149.11                                    \\ \hline
\begin{tabular}[c]{@{}c@{}}FSHNN \\ Obj Det \\ (6 layers STDP)\end{tabular} & 53.11             & $1.90 \times 10^8$   & 147.54                                    \\ \hline
\end{tabular}%
}
\end{table}


% \begin{figure}
%     \centering
%     \includegraphics[width = 0.5\linewidth]{Images/ee_map.png}
%     \caption{Figure Showing the plot for mAP vs Energy Advantage for Differenet Spiking Object Detectors}
%     \label{fig:my_label}
% \end{figure}


\subsection{Comparison to Spiking Yolo}


Here, we compare FSHNN model performance with the state-of-art spike-based object detector - Spiking YOLO \cite{kim2020spiking}. Though both of them are fully spiking object detectors, there are a few key differences in the two - firstly, the Spiking Yolo is made up only of backpropagated Spiking Convolution Layers which are trained using supervised learning. However, FSHNN couples both STDP based unsupervised learning methodologies with backpropagation learning. This helps the FSHNN network not only to achieve high performance and low uncertainty error but also to achieve properties like adversarial robustness. In addition to this, FSHNN also uses the MC Dropout method to calculate the uncertainty of the model, which further reinforces the robustness of the proposed architectural model. This is absent in the Spiking Yolo network which cannot estimate the uncertainty of the model. 
Also, the spiking YOLO object detector is based on YOLO architecture. However, YOLO suffers from an extreme class imbalance where the detectors evaluate a lot of extra candidate locations a majority of which do not contain an object. 
RetinaNet fixes this issue by using the Focal Pyramid Network and the Focal Loss. Hence, for this paper, we use RetinaNet as our base model. 
Similarly, for the spiking object detectors proposed in this paper, we see a significant increase in the observed mAP and mAR in the MS-COCO dataset. While the spiking YOLO reported an mAP of 26.24\%, the FSHNN network with 6 STDP layers described in this paper achieves $42.6\%$ which is higher than the mAP of the DNN based RetinaNet object detector.  %However, it must be noted that there is a significant difference in the architecture too - while the spiking Yolo is based solely on the backpropagated Spiking convolution layers, the FSHNN uses both supervised backpropagation and unsupervised STDP based learning methods, giving a much higher accuracy than the spiking 
Yolo. In addition to this, FSHNN also uses the MC Dropout method to calculate the uncertainty of the model, which further reinforces the robustness of the proposed architectural model.
 
However, it must also be noted that this comes at a cost - though our model has an energy advantage of around 150x compared to the DNN, it is comparatively larger than the Spiking YOLO network, which achieves an energy efficiency of 280x times the standard DNN.

\subsection{Results on the PASCAL-VOC Dataset}

To further show the generalizability of the model, we evaluate the model trained on the MS-COCO dataset on 5,823 frames from Pascal VOC \cite{everingham2010pascal},  which shares 20 object categories with the MS-COCO dataset. The results are shown in Table \ref{tab:pascal}. We see that though the performance of all the detectors is higher than that on the MS-COCO, the 6 layers STDP trained FSHNN object detector still outperforms the others.

\begin{table*}[]
\centering
\caption{Table showing the performance of the different object detectors on PASCAL VOC}
\label{tab:pascal}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c||c|}
\hline

& \textbf{mAP} & $\textbf{AP}_{S}$ & $\textbf{AP}_{M}$ & $\textbf{AP}_{L}$ & \textbf{mAR} & $\textbf{AR}_S$ & $\textbf{AR}_M$ & $\textbf{AR}_L$  & \textbf{mCMUE}\\ \hline
\textbf{RetinaNet}                                                          & 0.551       & 0.305        & 0.599        & 0.692        & 0.682       & 0.423        & 0.752        & 0.834    &  0.286    \\ \hline

\textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.526       & 0.278        & 0.564        & 0.668        & 0.648       & 0.401        & 0.707        & 0.801      &  0.301   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                      & 0.531       & 0.286        & 0.572        & 0.677        & 0.652       & 0.408        & 0.713        & 0.811     & 0.310   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                      &    0.573    &     0.318    &   0.622      &   0.731      &   0.684     &   0.419      &    0.749     &   0.823   &  0.293  \\ \hline
\end{tabular}%
}
\end{table*}



\subsection{Feature Fusion using STDP layers and Generalization}



\subsubsection{Generalizability of Object Proposal:} 

As described by Wang et al., \cite{wang2020leads} we define the generalizability of the object detector model to localize and not classify objects that are not annotated in the training dataset. For this experiment, we randomly split the MS-COCO dataset into two parts - the source dataset consisting of 70 classes and the target dataset consisting of 10 classes respectively. The source dataset consists of the set of seen classes and the target dataset consists of unseen classes. The target dataset is used to evaluate the generalization of the proposal model trained with the source dataset. For training, we use the train split and for evaluation, we use the 5000 images from the validation set. 

\textbf{Evluation Metric:} To evaluate the quality of the proposals, we use the standard average recall (AR@k) \cite{hosang2015makes}. One of the main motivations for building a generalized proposal model is to use the resulting proposals to train detection models for unseen classes with limited or no bounding box annotation.

\textbf{Implementation details:} We compare the generalization ability of the FSHNN based object detector and RetinaNet in Fig. \ref{fig:general}. The models are trained on the COCO-source-train dataset as described above. We report AR@100 on seen classes in the COCO-source-test dataset, as well as unseen classes in the COCO-target-test. We build on the hypothesis that the difference in performance between seen and unseen classes reflects the generalization gap. We also show an upper-bound performance on COCO-target-test obtained by models trained on the full training dataset containing both COCO-source-train and COCO-target-train. We notice that on seen classes, RetinaNet achieves a lower performance compared to FSHNN (a drop of 7.01\%). However, the drop is larger for unseen target classes (a drop of 11.9\%), indicating a larger generalization gap for RetinaNet. One reason for this is that RetinaNet is more sensitive to missing bounding boxes corresponding to unlabelled unseen classes in the source dataset. Proposals corresponding to unseen object classes that are not annotated in the training data are treated as hard-negatives, due to the use of focal-loss.  Hence,  the model heavily penalizes proposals corresponding to unannotated bounding boxes, leading to an overall drop in AR. Since some seen classes share visual similarity with unseen classes, this sensitivity to missing annotations affects AR for seen classes too.  However,  this effect is more magnified for unseen target classes.  
On the other hand, in FSHNN, only a small number of proposals that do not intersect with annotated bounding boxes are sampled at random as negatives. Hence, the probability that a proposal corresponding to an unseen object class is chosen as a negative is lower, leading to better generalization. 
Thus, we observe that the detection head of  FSHNN  provides better overall performance without sacrificing generalization. 



\begin{figure}
    \centering
    \includegraphics[width = 0.9\columnwidth]{Images/general.png}
    \caption{AR@100 corresponding to different models trained on COCO-source-train and evaluated on different test splits. Upper-bound corresponds to model trained on full COCO dataset and evaluated on COCO-target-test.}
    \label{fig:general}
\end{figure}

















==> Extras/related.tex <==
\section{Related Works}
\subsection{Object Detection:}

Object detection has become a critical problem of many computer vision tasks as it requires the estimation of both the category to which an object belongs and its spatial location. Recent work on Region-based  CNN  (R-CNN)  \cite{girshick2014rich} and its variants  like Fast RCNN \cite{girshick2015fast} Faster-RCNN \cite{ren2015faster}, MaskRCNN\cite{he2017mask} improves detection performance and speed. However, R-CNN-based networks suffer from a slow inference speed due to multiple-stage detection schemes and so, are not suitable for real-time object detection. As an alternative approach, one-stage detection methods have been proposed, where the bounding box information is extracted, and the objects are classified in a unified network. In  one-stage detection  models, Single-shot  multi-box  detector (SSD) \cite{liu2016ssd} and YOLO \cite{redmon2018yolov3} are notable. However, they achieve fast inference with the cost of lower mAP and mAR. Retinanet \cite{lin2017focal} overcomes these problems as it improves on the Faster-RCNN framework with the help of a focal loss and using ResNet+FPN as the backbone network to extract features. 

\subsection{Spiking Object Detection: }  Though object detection has been an important field of interest in computer vision, not much work has been done in the use of spiking neural networks based object detection. Recently, Kim et al. implemented a spiking version of the YOLO object detection architecture \cite{kim2020spiking}. They used channel-wise normalization and signed neuron with imbalanced threshold, to provide fast and accurate information transmission for deep SNNs. However, the proposed spiking YOLO object detector had a much lower performance compared to the standard DNN based YOLO and RetinaNet models.


\subsection{DNN-to-SNN conversion:}
Though SNNs offers a promise of low power deep learning models, they are still not widely popular mainly because their performance has not been comparable to their DNN counterparts and also scalability of spiking networks to large datasets. However, in recent years, to achieve higher accuracy, a promising approach has cropped up which converts DNNs trained with standard backpropagation into their spiking analog.
Recent works have proposed weight normalization and threshold balancing methods to obtain minimal loss in accuracy during the conversion process. In this paper, we use the threshold balancing method \cite{sengupta2019going} that gives near-lossless conversion performance for deep architectures like ResNet on complex Imagenet dataset.


\subsection{STDP based Unsupervised learning in SNN}
Spike Timing Dependent Plasticity (STDP) \cite{huang2014associative}, \cite{mcmahon2012stimulus} is a variant of the Hebbian unsupervised learning algorithm. This rule is proposed to describe the changes of a synaptic weight according to the relative timing of pre and post-synaptic spikes. In STDP, if a presynaptic spike precedes a postsynaptic spike, a synaptic weight is potentiated.

If the time interval between the pre-and postsynaptic spike is $t=t_{\text {post}}-t_{\text {pre}}$ and $\mathrm{t}>0$ then the synaptic weight will be potentiated. The magnitude of the potentiation is a function of t which decays exponentially with a time constant $\tau_{+}$ and can be calculated by $\mathrm{A}_{+} \mathrm{e}^{-\mathrm{t} / \tau_{+}},$ where $\mathrm{A}_{+}$ is the maximum synaptic change. Alternatively, the synaptic efficacy decreases if a presynaptic spike occurs shortly after the postsynaptic one. The magnitude of the decrease can be calculated by $\mathrm{A}_{-} \mathrm{e}^{\mathrm{t} / \tau_{-}},$ where $\mathrm{A}_{-}$ represents the maximum depression, and $\tau_{-}$ is a time constant. 

There are various spiking neural networks (SNNs) to solve object recognition and image classification tasks by converting the traditional DNNs into spiking networks by replacing each DNN computing unit with a spiking neuron \cite{cao2015spiking,diehl2016conversion, hunsberger2015spiking}. These networks aim to reduce the energy consumption in DNNs while achieving a similar accuracy score. 




\subsection{Backpropagation based Supervised Learning in SNN} 

 Backpropagation-based supervised learning for spiking neural networks has played a critical role in improving their performance. %Zenke et al. \cite{zenke2018superspike} proposed a voltage based gradient descent approach to train multilayer network to process spatiotemporal spiking patterns. Mostafa et al. \cite{pedroni2018small} on the other hand, used nonleaky integrate-and-fire neurons for a backpropagation learning method for SNNs composed of multiple layers.
 A major setback for using backpropagation based method for spiking neural networks was the non-differentiability of spike-based backpropagation methods of spiking neurons.
 However, several recent works have addressed the issue in different ways. While Huh et al. approximated the spiking neuron model as continuous and differentiable \cite{huh2018gradient}, other works defined the surrogate gradient as the continuous approximation of the real gradient\cite{wu2018spatio, neftci2019surrogate}. 
Rathi et. al uses a hybrid training technique that combines ANN-SNN conversion and spike-based BP that reduces the latency and helps in better convergence \cite{rathi2020enabling}.  The authors use the ANN-SNN conversion as an initialization step followed by spike-based backpropagation (STDB) incremental training. The authors also demonstrated the approach of taking a converted SNN and incrementally training it using backpropagation. This hybrid approach improves the energy-efficiency and accuracy compared to standard models trained with either only spike-based backpropagation or only converted weights.




\subsection{Generalizability of Neural Networks}

Recent works \cite{jacot2018neural, huang2020deep, chen2020generalized} have analyzed overparameterized (wide) neural networks from a theoretical perspective by connecting them to reproducing kernel Hilbert spaces. They also proved that under proper conditions, the weight matrices of a well-trained overparameterized (achieving any given small training error) are very close to their initialization. Thus, during training the model searches within some class of reproducing kernel functions, where the associated kernel is called the “neural tangent kernel” which only depends on the initialization of the weights. Accordingly, the generalization properties of the overparameterized neural network are equivalent to those of the associated NTK function class.
Alternatively, another line of research \cite{csimcsekli2020hausdorff} has worked on comparing the generalization error while using different training strategies. In the paper, the authors show that we can control the generalization error of a training algorithm using the Hausdorff dimension of its trajectories. The authors further evaluated the generalization error of the SGD process that is characterized by the Feller process, though the results can easily be generalized to other stochastic processes. 
Again, in recent literature the notion of generalizability is measured by either of the three notions: (i) the \textit{flatness} of the local minimum found by SGD, which is related to the eigenvalues of the Hessian, (ii) the \textit{ratio of the stepsize $\eta$ to the batch size $b$}, that controls the magnitude of the stochastic gradient noise, and (iii) the \textit{tail-index}, which measures the heaviness of the tails of the network weights at convergence. In \cite{gurbuzbalaban2020heavy}, the authors showed that these concepts are inherently interlinked and showed that depending on the structure of the Hessian of the loss at the minimum, and the choices of the algorithm parameters $\eta, b$, the SGD iterates will converge to a heavy-tailed stationary distribution.



Recent works have worked on determining the generalization characteristics of the object proposal generation that is the first step in detection models \cite{wang2020leads}. 
A more generalizable object proposal can help to scale detection models to a larger number of classes with fewer annotations. Motivated by this, the authors study how a detection model trained on a small set of source classes can provide proposals that generalize to unseen classes.  



==> Extras/results.tex <==
Table 5:



\begin{table}[]
\centering
\caption{Table Describing the Learning Blocks used in the Architectures}
\label{tab:layers}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 &  & \textbf{Block 1} & \textbf{Block 2} & \textbf{\begin{tabular}[c]{@{}c@{}}ResNet\\ Block\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FPN\\  Block\end{tabular}} \\ \hline
\multirow{2}{*}{\textbf{Retinanet}} & Layer & None & None & CNN & CNN \\ \cline{2-6} 
 & Learning & N/A & N/A & BP & BP \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN \\ Obj Det\end{tabular}}} & Layer & SNN & SNN & SNN & SNN \\ \cline{2-6} 
 & Learning & BP & STDP & BP & BP \\ \hline

\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking\\  Obj Det\end{tabular}}} & Layer & SNN & SNN & SNN & SNN \\ \cline{2-6} 
 & Learning & BP & BP & BP & BP \\ \hline
\end{tabular}%
}
\end{table}











Table 3:
\begin{table*}[]
\centering
\caption{Table showing Performance of the FSHNN based Object Detector with Increasing STDP Layers}
\label{tab:abl1}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c||c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Number of \\ STDP Layers\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Classification\\  Loss\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Regression \\ Loss\end{tabular}} &  \textbf{mAP} & $\textbf{AP}_{S}$ & $\textbf{AP}_{M}$ & $\textbf{AP}_{L}$ & \textbf{mAR} & $\textbf{AR}_S$ & $\textbf{AR}_M$ & $\textbf{AR}_L$  & \textbf{mCMUE}\\ \hline 

\textbf{3}                                                               & 0.4127                                                                      & 0.6912                                                                  & 0.379  & 0.198 & 0.407 &  0.482   & 0.492    & 0.292 & 0.554 & 0.615  & 0.251 \\ \hline
\textbf{4}                                                               & 0.3841                                                                      & 0.6787                                                                  & 0.392  & 0.203 & 0.425 &  0.507  & 0.515    &  0.308 & 0.578 &  0.635 & 0.244 \\ \hline
\textbf{5}                                                               & 0.3352                                                                      & 0.6536                                                                  & 0.409    & 0.211 & 0.439 &  0.518 & 0.527   & 0.316 & 0.591 & 0.652   & 0.236 \\ \hline
\textbf{6}                                                               & 0.3076                                                                      & 0.6193                                                                  & 0.426   & 0.229 & 0.452 & 0.533  & 0.541    & 0.327 & 0.612 & 0.668 & 0.229 \\ \hline
\end{tabular}
\end{table*}


Table 3 edited:

\begin{table*}[]
\centering
\hlt{
\caption{\hlt{Table showing Performance of the FSHNN based Object Detector with Increasing STDP Layers}}
\label{tab:abl1}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c||c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Number of \\ STDP Layers\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Classification\\  Loss\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Regression \\ Loss\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}}mAP \\ (mean $\pm$ var) \end{tabular}} & $\textbf{AP}_{S}$ & $\textbf{AP}_{M}$ & $\textbf{AP}_{L}$ & \textbf{\begin{tabular}[c]{@{}c@{}}mAR \\ (mean $\pm$ var) \end{tabular}} & $\textbf{AR}_S$ & $\textbf{AR}_M$ & $\textbf{AR}_L$  & \textbf{\begin{tabular}[c]{@{}c@{}}mean \\ mCMUE \end{tabular}}\\ \hline 

\textbf{3}                                                               & 0.4127                                                                      & 0.6912                                                                  &  0.377 $\pm 0.0423$
  & 0.198 & 0.407 &  0.482   & $0.490 \pm 0.0467$    & 0.292 & 0.554 & 0.615  & 0.251 \\ \hline
\textbf{4}                                                               & 0.3841                                                                      & 0.6787                                                                  & $0.391 \pm 0.0411$  & 0.203 & 0.425 &  0.507  & $0.511 \pm 0.0431$    &  0.308 & 0.578 &  0.635 & 0.244 \\ \hline
\textbf{5}                                                               & 0.3352                                                                      & 0.6536                                                                  & $0.406 \pm 0.0397$    & 0.211 & 0.439 &  0.518 & $0.523 \pm 0.0410$   & 0.316 & 0.591 & 0.652   & 0.236 \\ \hline
\textbf{6}                                                               & 0.3076                                                                      & 0.6193                                                                  & $0.420 \pm 0.0399$   & 0.229 & 0.452 & 0.533  & $0.537 \pm 0.0403$     & 0.327 & 0.612 & 0.668 & 0.229 \\ \hline
\end{tabular}
}
\end{table*}


Table 4:


\begin{table}[]
\centering
\caption{Table showing Robustness of FSHNN based Object Detector for Noisy Testing Data and Limited Labelled Training Dataset }
\label{tab:abl2}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}\# of STDP\\ Layers\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Classification\\  Loss\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Regression \\ Loss\end{tabular}} & \textbf{mAP} & \textbf{mAR} & \textbf{cMUE}  \\ \hline
\multicolumn{6}{|c|}{\textbf{SNR = 30dB}}                                                                                                                                                                                                                              \\ \hline
\textbf{3}                                                               & 0.4318                                                                      & 0.7165                                                                  & 0.368        & 0.483        & 0.317 \\ \hline
\textbf{4}                                                               & 0.3987                                                                      & 0.7093                                                                  & 0.382        & 0.497        & 0.305 \\ \hline
\textbf{5}                                                               & 0.3516                                                                      & 0.6845                                                                  & 0.395        & 0.519        & 0.291 \\ \hline
\textbf{6}                                                               & 0.3204                                                                      & 0.6522                                                                  & 0.412        & 0.531        & 0.284 \\ \hline
\multicolumn{6}{|c|}{\textbf{SNR = 15dB}}                                                                                                                                                                                                                              \\ \hline
\textbf{3}                                                               & 0.6723                                                                      & 0.7345                                                                  & 0.305        & 0.441        & 0.455 \\ \hline
\textbf{4}                                                               & 0.6552                                                                      & 0.7269                                                                  & 0.316        & 0.453        & 0.448 \\ \hline
\textbf{5}                                                               & 0.6218                                                                      & 0.7114                                                                  & 0.324        & 0.465        & 0.439 \\ \hline
\textbf{6}                                                               & 0.6014                                                                      & 0.7008                                                                  & 0.331        & 0.476        & 0.431 \\ \hline
\hline
\multicolumn{6}{|c|}{\textbf{80\% Training Data}}                                                                                                                                                                                                                               \\ \hline
\textbf{3}                                                               & 0.4157                                                                      & 0.6998                                                                  & 0.358        & 0.473        & 0.301 \\ \hline
\textbf{4}                                                               & 0.3806                                                                      & 0.6742                                                                  & 0.363        & 0.481        & 0.289 \\ \hline
\textbf{5}                                                               & 0.3694                                                                      & 0.6516                                                                  & 0.392        & 0.514        & 0.214 \\ \hline
\textbf{6}                                                               & 0.3356                                                                      & 0.6288                                                                  & 0.411        & 0.547        & 0.199 \\ \hline
\multicolumn{6}{|c|}{\textbf{60\% Training Data}}                                                                                                                                                                                                                               \\ \hline
\textbf{3}                                                               & 0.4975                                                                      & 0.7884                                                                  & 0.329        & 0.431        & 0.390 \\ \hline
\textbf{4}                                                               & 0.4698                                                                      & 0.7545                                                                  & 0.348        & 0.476        & 0.358 \\ \hline
\textbf{5}                                                               & 0.4513                                                                      & 0.7312                                                                  & 0.364        & 0.493        & 0.317 \\ \hline
\textbf{6}                                                               & 0.4027                                                                      & 0.7084                                                                  & 0.396        & 0.518        & 0.296 \\ \hline
\multicolumn{6}{|c|}{\textbf{40\% Training Data}}                                                                                                                                                                                                                               \\ \hline
\textbf{3}                                                               & 0.6057                                                                      & 0.9432                                                                  & 0.287        & 0.386        & 0.513 \\ \hline
\textbf{4}                                                               & 0.5964                                                                      & 0.9303                                                                  & 0.296        & 0.401        & 0.501 \\ \hline
\textbf{5}                                                               & 0.5837                                                                      & 0.9268                                                                  & 0.308        & 0.415        & 0.486 \\ \hline
\textbf{6}                                                               & 0.5759                                                                      & 0.9115                                                                  & 0.322        & 0.426        & 0.478 \\ \hline
\end{tabular}
\end{table}

Table 6:

\begin{table*}[]
\centering
\caption{Table showing the performance of the different object detectors}
\label{tab:perf_comp}
\resizebox{0.65\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c||c|}
\hline

& \textbf{mAP} & $\textbf{AP}_{S}$ & $\textbf{AP}_{M}$ & $\textbf{AP}_{L}$ & \textbf{mAR} & $\textbf{AR}_S$ & $\textbf{AR}_M$ & $\textbf{AR}_L$  & \textbf{mCMUE}\\ \hline
\multicolumn{10}{|c|}{\textbf{No Noise; 100\% Training Data}}                                                                                                                                                           \\ \hline
\textbf{RetinaNet}                                                          & 0.388       & 0.207        & 0.420        & 0.498        & 0.501       & 0.301        & 0.566        & 0.624    &  0.237    \\ \hline

\textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.375       & 0.189        & 0.401        & 0.477        & 0.486       & 0.283        & 0.549        & 0.598      &  0.254   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                      & 0.379       & 0.198        & 0.407        & 0.482        & 0.492       & 0.292        & 0.554        & 0.615     & 0.251   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                      &    0.426    &     0.223    &   0.452      &   0.526      &   0.541     &   0.312      &    0.611     &   0.682   &  0.229  \\ \hline
\end{tabular}%
}
\end{table*}

Table 7:
\begin{table*}[]
\centering
\caption{Table showing the performance of the different object detectors with input noise during testing}
\label{tab:comp_noise}
\resizebox{0.65\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c||c|}
\hline

& \textbf{mAP} & $\textbf{AP}_{S}$ & $\textbf{AP}_{M}$ & $\textbf{AP}_{L}$ & \textbf{mAR} & $\textbf{AR}_S$ & $\textbf{AR}_M$ & $\textbf{AR}_L$  & \textbf{mCMUE}\\ \hline

\multicolumn{10}{|c|}{\textbf{SNR = 30dB}}                                                                                                                                                         \\ \hline
\textbf{RetinaNet}                                                          & 0.371       & 0.183        & 0.409        & 0.481        & 0.489       & 0.279        & 0.554        & 0.613   & 0.313  \\ \hline

\textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.365       & 0.186        & 0.388        & 0.472        & 0.478       & 0.278        & 0.543        & 0.589       & 0.320 \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                      & 0.368       & 0.190        & 0.395        & 0.476        & 0.483       & 0.285        & 0.549        & 0.605       & 0.317   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                      &  0.412      &   0.211      &   0.446      &       0.482  &     0.531   &  0.308       &  0.599        &    0.668    &  0.284  \\ \hline
\multicolumn{10}{|c|}{\textbf{SNR = 15dB}}                                                                                                                                                         \\ \hline
\textbf{RetinaNet}                                                          & 0.277       & 0.104        & 0.237        & 0.349        & 0.416       & 0.204        & 0.401        & 0.426       & 0.605  \\ \hline

\textbf{\begin{tabular}[c]{@{}c@{}}BP Spiking \\ Obj Detector\end{tabular}} & 0.297       & 0.159        & 0.347        & 0.406        & 0.428       & 0.248        & 0.473        & 0.539       & 0.483  \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (3 STDP layers)\end{tabular}}                                                     & 0.305       & 0.163        & 0.358        & 0.417        & 0.441       & 0.257        & 0.496        & 0.553     & 0.455   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}FSHNN Obj Det \\  (6 STDP layers)\end{tabular}}                                                    &   0.331     &   0.184      &    0.392     &   0.451      &    0.476     &    0.271    &    0.528     &  0.587    &  0.431  \\ \hline

\end{tabular}%
}
\end{table*}





Table 11:
\begin{table*}[]
\centering
\hlt{
\caption{\hlt{Table showing Performance Comparison of the FSHNN based Object Detector with respect to other Hybrid Models}}
\label{tab:abl1}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Number of \\ STDP Layers\end{tabular}} &  \textbf{mAP} & $\textbf{AP}_{S}$ & $\textbf{AP}_{M}$ & $\textbf{AP}_{L}$ & \textbf{mAR} & $\textbf{AR}_S$ & $\textbf{AR}_M$ & $\textbf{AR}_L$  \\ \hline 

\textbf{3 layer STDP FSHNN}                                                                                                                    & 0.379   & 0.198 & 0.407 &  0.482   & 0.492    & 0.292 & 0.554 & 0.615 \\ \hline
\textbf{6 layer STDP FSHNN}                                                                                                                    & 0.426   & 0.229 & 0.452 & 0.533  & 0.541    & 0.327 & 0.612 & 0.668  \\ \hline
\textbf{BP Spiking  Obj Det} & 0.375       & 0.189        & 0.401        & 0.477        & 0.486       & 0.283        & 0.549        & 0.598   \\ \hline
\textbf{Large STDP FSHNN}                                                                                                                     & 0.268   & 0.119 & 0.284 & 0.356  & 0.376    & 0.195 & 0.396 & 0.489  \\ \hline
\textbf{Small STDP FSHNN}                                                                                                                     & 0.251   & 0.106 & 0.279 & 0.348  & 0.369    & 0.190 & 0.387 & 0. 481 \\ \hline
\textbf{Hybird UCSN Obj Det}                                                                                                                   & 0.383   & 0.191 & 0.411 & 0.487  & 0.497    & 0.290 & 0.559 & 0.621  \\ \hline
\textbf{Hybrid CAE Obj Det}                                                                                                                   & 0.381   & 0.189 & 0.415 & 0.486  & 0.500    & 0.289 & 0.561 & 0.627  \\ \hline
\end{tabular}
}
\end{table*}


==> tex/abstract.tex <==
\begin{abstract}
% Over the last few decades Deep Neural Networks (DNNs) have been widely used to solve various complex tasks like image classification, object recognition and object detection. Of these, object detection has been of keen interest of researchers due to its application in varied fields like self-driving cars. However, as the complexity of the problem increases, there is an increase in the demand of computational and consequently power resources for such problems. In order to achieve a on-board computation, such resource constraints may impose a challenge. Also, modern DNNs have some very important setbacks - firstly, they require an exorbitant amount of data to train and perform very poorly on noisy input data. In this paper, we propose a Hybrid Learning based Fully Spiking Object Detector which combines STDP based unsupervised learning with back propagation learning. We observe that this new model solves the key issues in current DNNs - it performs much better than the standard DNN with limited labelled training data and also noisy data, while giving comparable AP and AR to the standard DNN for the standard cases. We evaluated our model on the MS COCO dataset and observed that it consumes almost 300 times less energy compared to its DNN counterpart. 

% Object detection has been an area of keen interest of researchers due to its application in varied fields like self-driving cars. However, as the complexity of the problem increases, there is an increase in the demand of computational and consequently power resources for such problems for Deep Neural Network (DNN) based object detectors. Spiking Neural Networks (SNNs) offers an energy-efficient alternative for implementing deep learning applications by making use of asynchronous discrete events or spikes. In addition to this, current state-of-the-art DNNs perform poorly when subjected to adversarial conditions like less training data or noisy test data. In this paper, we propose a novel hybrid learning based fully spiking robust object detector. We use a novel training methodology which combines STDP based unsupervised learning with incremental spike-timing dependent backpropagation (STDB) learning. We observe that this new model outperforms the current state-of-the-art object detectors when subjected to the adversarial conditions, while giving comparable AP and AR to the standard DNN for the standard cases. Our evaluation of the model on the MS COCO dataset showed that it consumes almost 300 times less energy compared to its DNN counterpart.

%  Spiking Neural Networks (SNNs) offers an energy-efficient alternative for implementing deep learning applications by making use of asynchronous discrete events or spikes. In this paper, we propose a novel hybrid learning based fully spiking robust object detector. We use a hybrid training methodology which combines synaptic time dependent plasticity (STDP) based unsupervised learning technique with incremental spike-timing dependent backpropagation (STDB) learning method. We levarage the current advancements in DNN-to-SNN conversion techniques to get a spiking neural network model from a DNN based model and then augment the obtained model with frozen trained STDP layers to get the final neural network. Hence, we use the weights and thresholds obtained from the coversion step as an initialization point for STDB to get the final trained model. This model outperforms the current state-of-the-art DNN based object detectors when subjected to adversarial conditions,like less training data or noisy test data, while giving comparable AP and AR to the standard DNN for the standard cases. Our evaluation of the model on the MS COCO dataset showed that it consumes almost 300 times less energy compared to its DNN counterpart.

This paper proposes a Fully Spiking Hybrid Neural Network (FSHNN) for energy-efficient and robust object detection in resource-constrained platforms. The network architecture is based on Convolutional SNN using leaky-integrate-fire neuron models. The model combines unsupervised Spike Time-Dependent Plasticity (STDP) learning with back-propagation (STDB) learning methods and also uses Monte Carlo Dropout to get an estimate of the uncertainty error. FSHNN provides better accuracy compared to DNN based object detectors while being 150X energy-efficient. It also outperforms these object detectors, when subjected to noisy input data and less labeled training data with a lower uncertainty error.% of the proposed model in these operations is significantly lower compared to its DNN and other SNN counterparts that further reinforces the robustness of the proposed model.

\end{abstract}
\begin{IEEEkeywords}
Uncertainty Estimation, Neural Architecture Search, Monte Carlo Dropout, DARTS, ImageNet, Image classification.
\end{IEEEkeywords}

